Pushing Test-Time Scaling Limits of Deep Search with Asymmetric Verification

Test-time compute can be scaled both sequentially and in parallel. Sequential scaling involves lengthening the generation process, while parallel scaling involves verifying and selecting among multiple candidate outputs. Combining these two strategies has led to the most powerful AI systems, such as Grok 4 Heavy and GPT-5 Pro. In certain contexts (e.g., solving Sudoku puzzles), verifying responses can be substantially easier than generating them. This property, referred to as \emph{asymmetric verification}, highlights the strong potential of test-time scaling (TTS). In this work, we study both sequential and parallel TTS of deep search agents, motivated by the intuition that verification in this setting is often much easier than generation. In experiments, we first show that sequential scaling methods, such as budget forcing, can be effective initially but soon degrade performance. Leveraging asymmetric verification, however, we are able to achieve substantial improvements by allocating only a modest amount of compute to the verifier. We conduct experiments with flagship open-source models and extend them to their ``Heavy'' variants through TTS. These deep research agents achieve gains of up to 27 absolute points on benchmarks such as BrowseComp. Remarkably, as an open-source alternative, GLM-4.5 Heavy reaches accuracy of {\bf 54.0\%} on BrowseComp and {\bf 66.0\%} on GAIA, placing it comparable to the best proprietary choices such as OpenAI Deep Research. Tongyi-DeepResearch Heavy further achieves {\bf 69.0\%} accuracy on BrowseComp, greatly surpassing the best proprietary results.

==> Introduction.tex <==


% \begin{figure}[!t]
%         \centering
% \includegraphics[width=0.99\columnwidth]{iclr2026/fig/fig1_merged_v2.pdf}
% \vspace{-10pt}
% \caption{Figure 1.}
%         \label{fig:figure1}
%         \vspace{-10pt}
% \end{figure}

% \begin{figure}[!b]
% \vspace{-10pt}
%         \centering
% \includegraphics[width=0.95\textwidth]{iclr2026/fig/Figure1-15_5.pdf}
% \vspace{-10pt}
% \caption{The top part shows performance on BrowseComp and GAIA. Results marked with * are from our test runs; \emph{*-Heavy} denotes the performance after test-time scaling. The bottom left shows how accuracy on BrowseComp varies with test-time compute represented by the number of tool calls. Solid lines indicate scaling the compute of the search agent, and dashed lines indicate allocating additional compute to a verifier agent. The bottom right shows strategies for extending GLM-4.5 to a ``Heavy Variant'' on BrowseComp, including sequential scaling, parallel scaling of the search agent, and scaling the verifier's compute.
%         }
%         \label{fig:figure1}
%     %\vspace{-10pt}

% \end{figure}
% \jh{Plz revise intro according to the updated abstract}
% Advanced proprietary Deep Research systems—such as OpenAI Deep Research~\citep{openai2025deepresearch}, Gemini Deep Research~\citep{google2025geminideepresearch}, and Grok DeepSearch~\citep{xai2025grok3beta}—can autonomously search the web, browse hundreds or even thousands of pages, synthesize the gathered information, and produce comprehensive reports rivaling those of human research analysts. A defining strength of these systems is their powerful test-time scaling\citep{snell2024scaling,muennighoff2025s1}: for complex research tasks, they can execute extended multi-step plans, spending hours collecting data and identifying gaps—where more compute time typically yields better results. Unlike traditional reasoning models, which excel mainly in constrained domains such as coding or mathematics\citep{jaech2024openai,team2025kimi,seed2025seed1}, Deep Research systems operate in open-ended, real-world environments, combining reasoning with active information gathering to solve problems that cannot be addressed from internal knowledge alone.

\begin{figure}[h]
\vspace{-15pt}
        \centering
    \begin{minipage}{0.96\textwidth}
    \centering
        \subfigure{
                \includegraphics[width=0.48\textwidth]{iclr2026/fig/fig11.pdf}
        }
        \hfill
        \subfigure{
                \includegraphics[width=0.48\textwidth]{iclr2026/fig/fig12.pdf}
        }
    \end{minipage}
    \vspace{-10pt}
 \subfigure{  
\includegraphics[width=0.96\textwidth]{iclr2026/fig/Figure18_12.pdf}}
% \vspace{-8pt}
\caption{\textbf{Top part} shows accuracy on BrowseComp and GAIA. Results marked with * are from our test runs; \emph{*-Heavy} denotes the accuracy after our test-time scaling. \textbf{Bottom left} shows how accuracy on BrowseComp varies with tool calls. Solid lines indicate scaling the search agent’s compute, dashed lines indicate allocating compute to a verifier. \textbf{Bottom right} shows strategies for extending GLM-4.5 to GLM-4.5 Heavy on BrowseComp.
% , including sequential scaling, parallel scaling of the search agent, and scaling the verifier's compute.
        }
        \label{fig:figure1}
    % \vspace{-10pt}

\end{figure}

\section{Introduction}
Test-time scaling underpins the progress of most advanced AI systems, such as Grok 4 Heavy~\citep{xai2025grok4}, GPT-5-Thinking-Pro~\citep{openai2025gpt5systemcard}, and  Gemini 2.5 Pro~\citep{deepmind2025gemini2_5pro}. It operates through two complementary strategies~\citep{snell2024scaling}: sequential scaling and parallel scaling. Sequential scaling deepens reasoning by extending chains of thought, as in OpenAI-o1~\citep{jaech2024openai}, DeepSeek-R1~\citep{guo2025deepseek}, and Kimi-k1.5~\citep{team2025kimia}, where reinforcement learning encourages reflective reasoning that can unravel complex tasks. Parallel scaling, by contrast, broadens the exploration space by producing multiple candidate outputs and selecting among them through aggregation methods such as Best-of-K selection. This strategy is widely used in advanced closed-source systems such as GPT-5-Thinking-Pro~\citep{openai2025gpt5systemcard} and Gemini-2.5 Pro~\citep{deepmind2025gemini2_5pro}. While expanding exploration space greatly increases the likelihood of capturing the correct solution, it also imposes steep computational costs.

%While this significantly increases the chance of covering the correct solution, it does so at steep computational cost.

%\jh{i removed discussion on majority voting as it is not a general approach for open generation, and it is not really used in practice for actual systems}
% Moreover, simple methods like majority voting exhibit diminishing returns: as the number of sampled trajectories increases, performance eventually saturates—or even declines~\citep{chen2024more,fu2025deep}.

% \jh{this paragraph needs rewriting, plz see the abstract. It is not like ``previous work explore tts for code/math, while we explore tts for a new domain'' -- this sounds too superficial and not well-motivated. As shown in the abstract, let's directly start talking about verification of TTS and asymmetric verification, and then we introduce agentic search as an important domain and it may well-suite asymmetric verification, which is why we decide to study TTS for agentic search}

Compared to spending test-time compute on endlessly expanding the number of candidate outputs, allocating compute to verification to evaluate and select outputs introduces a new and orthogonal scaling dimension. Many tasks, such as Sudoku, exhibit an \emph{Asymmetry of Verification}~\citep{wei2025asymmetry}: they are far easier to verify than to solve, meaning that allocating compute to verifiers may yield disproportionate benefits. Many applications of deep search are prime examples of this property. In deep search, the models are often required to search deeply over the web through multiple recursive searching operations, browse hundreds or even thousands of pages, and identify information that satisfies the users' needs.
% autonomously search the web, browse hundreds or even thousands of pages, synthesize information, and produce comprehensive reports \jhc{rivaling those of human analysts—ultimately freeing knowledge workers from time-intensive tasks}{}~\citep{openai2025deepresearch,google2025geminideepresearch,xai2025grok3beta}. 
In such scenarios, forward search must navigate an enormous, sparsely informative space, while backward verification begins with a candidate answer and checks whether it satisfies well-defined conditions~\citep{wei2025browsecomp}, drastically shrinking the search space and making far more efficient use of compute. Research on test-time scaling for deep search, particularly leveraging this asymmetry, therefore opens the path to building powerful and cost-effective agentic search systems such as Deep Research~\citep{openai2025deepresearch,google2025geminideepresearch,xai2025grok3beta}. 


% Previous work on test-time scaling has largely focused on narrow reasoning domains such as coding and mathematics~\citep{muennighoff2025s1,luo2025deepscaler}, where extending the number of ``thinking tokens'' reliably boosts performance. By contrast, research on deep research systems remains limited. These systems operate in open-ended, real-world settings where solving problems requires not only reasoning but also active information gathering—retrieving, evaluating, and integrating evidence that cannot be derived from internal knowledge alone~\citep{openai2025deepresearch,google2025geminideepresearch,xai2025grok3beta}. In this context, scaling means more than generating longer reasoning chains: it involves executing additional actions, interacting with external environments, and processing retrieved observations. A further challenge is that deep research deep research unfolds within an enormous and sparsely informative search space, implementing test-time scaling—particularly parallel scaling—can be computationally expensive. Nevertheless, deep research tasks possess an important property: \emph{asymmetric verification} \citep{wei2025asymmetry}. While generating a correct solution is often difficult, verifying a proposed answer can be far easier. Despite its potential to reshape scaling strategies, this property remains underexplored.



% \begin{figure}[!t]
%         \centering
% \includegraphics[width=0.99\columnwidth]{iclr2026/fig/fig1_merged_v2.pdf}
% \vspace{-10pt}
% \caption{Figure 1.}
%         \label{fig:figure1}
%         \vspace{-10pt}
% \end{figure}


% \begin{figure}[htbp]
% \vspace{-10pt}
%         \centering
% \includegraphics[width=0.98\textwidth]{iclr2026/fig/fig1_merged_v2.pdf}
% \vspace{-10pt}
% \caption{Figure 1.
%         }
%         \label{fig:figure1}
%     \vspace{-10pt}

% \end{figure}

% Recent open-source efforts have attempted to replicate these systems, often training models via reinforcement learning to handle multi-round interactions with search engines~\citep{jin2025search,zheng2025deepresearcher}. However, these approaches typically involve only a few interaction rounds and focus on relatively simple tasks—such as HotpotQA~\citep{yang2018hotpotqa}—that models can often solve using internal knowledge. Other pipelines combine supervised fine-tuning on synthetic data with reinforcement learning to instill more complex browsing behaviors~\citep{li2025websailor,shi2025pangu}, yet performance on challenging web-browsing benchmarks such as BrowseComp~\citep{wei2025browsecomp} remains low, with accuracy rarely exceeding 15\%.


% \begin{figure}[!t]
%         \centering
% \includegraphics[width=0.99\columnwidth]{iclr2026/fig/fig1_merged_v2.pdf}
% \vspace{-10pt}
% \caption{Figure 1.}
%         \label{fig:figure1}
%         \vspace{-10pt}
% \end{figure}


% Crucially, most prior work focuses on scaling training compute, leaving open the question of whether comparable or superior capabilities can be achieved by scaling test-time compute instead. For reasoning models, increasing thinking tokens can substantially improve results in coding or mathematics~\citep{muennighoff2025s1,deepcoder2025}, but agentic systems pose a different challenge: scaling involves not just longer reasoning but more actions, interactions with external environments, and processing of retrieved observations. Whether scaling test-time compute in such interactive settings produces qualitatively new behaviors or significant performance gains remains unclear.

% In this work, we use the deep search capabilities of Deep Research systems as a representative case to study how scaling test-time compute affects complex information-seeking behavior. We build a simple yet effective agentic scaffold and first scale the computation available to search agents, revealing a key inefficiency: even with generous tool usage quotas, models do not proportionally increase search tool usage. Instead, usage growth slows while performance drops sharply. Inspired by~\citet{muennighoff2025s1}, we propose \emph{budget forcing}—granting extra computation when the model ends a task prematurely and prompting exploration of alternative solution paths. This substantially boosts tool usage and Pass@1 accuracy: GLM-4.5 improves from 0.19 to 0.27, and Qwen3-0527 from 0.08 to 0.18 on BrowseComp-en. We then study \emph{parallel scaling}, a method widely used in advanced closed-source systems such as GPT-5-Thinking-Pro~\citep{openai2025gpt5systemcard} and Gemini 2.5 Pro~\citep{deepmind2025gemini2_5pro}. Parallel compute expansion further strengthens exploration: GLM-4.5 achieves 60\% pass@16 on BrowseComp-en. However, these gains expose a critical bottleneck: scaling compute broadens the search space but does not help the search agent effectively identify the best candidates—pointing to the need to shift compute from exploration toward exploitation.

In this work, we use the deep search capabilities of Deep Research systems as a representative case to study how scaling test-time compute affects complex information-seeking behavior. Under a simple agentic scaffold, we first investigate strategies that encourage models to increase search tool usage within a single trajectory. For example,
%Under a simple agentic scaffold, we first scale the computation allowable to the search agent by increasing the maximum number of tool calls, which reveals a key inefficiency: even with generous tool usage quotas, models do not proportionally increase search tool usage. Instead, usage growth slows while performance drops sharply. 
we adopt the \emph{budget forcing} strategy of~\citet{muennighoff2025s1}. By forcing models to make additional tool calls after premature termination, we incentivize exploration of alternative reasoning paths.
% Inspired by~\citet{muennighoff2025s1}, we propose \jh{it is not proposed by us}\emph{budget forcing}—granting extra computation when the model ends a task prematurely and prompting exploration of alternative solution paths.
This substantially boosts tool usage and Pass@1 accuracy: GLM-4.5~\citep{zeng2025glm} improves from 19\% to 27\%, and Qwen3-0527 from 8\% to 18\% on the challenging BrowseComp benchmark~\citep{wei2025browsecomp}. However, excessive budget forcing eventually degrades performance. To address this, we turn to \emph{parallel scaling}, where expanding compute in parallel further strengthens exploration: GLM-4.5 achieves 67\% Pass@32 accuracy on BrowseComp. However, these gains expose a critical bottleneck: scaling compute broadens the search space but does not help the search agent effectively identify the best candidates—pointing to the need to shift compute from search toward verification. 


% The \emph{Asymmetry of Verification}~\citep{wei2025asymmetry} offers exactly such a shift.

%describing tasks where verifying a solution is far easier than generating it. 
% Deep search tasks embody this property: forward search requires navigating an enormous, sparsely informative space, whereas backward verification starts from a candidate answer and simply checks whether it meets specific conditions—drastically reducing the search space and improving compute exploitation. 
Deep search benefits from this shift because of the \emph{Asymmetry of Verification}, where verifying an answer may be much easier than generating one.
For instance, on BrowseComp, GLM-4.5 needs about 75 search tool calls on average to solve a problem, but verifying a candidate answer requires only about 18 tool calls. We leverage this asymmetry by adapting the search agent into a verifier agent with minimal modifications, which produces substantial efficiency gains (see Figure~\ref{fig:figure1} bottom left). On BrowseComp, scaling search agent alone is costly: for GLM-4.5, raising accuracy from 30\% to 40\% requires roughly 500 additional tool calls. In contrast, adding a verifier achieves the same 10-point accuracy increase with only about 100 extra calls. Moreover, verifier performance scales well with additional compute, where budget forcing and parallel sampling further improve the accuracy on filtering correct answers.


% We adapt the search agent into a verifier agent with minimal changes, yielding large efficiency gains as shown in Figure~\ref{fig:figure1}: on BrowseComp, GLM-4.5 scores around 30\% with \emph{maj@8} (majority vote from 8 candidates), but achieves 40\% using a \emph{weighted-of-8} scheme that ranks candidates by verifier-assigned confidence—requiring only one-quarter to one-third of the compute needed to match this improvement through further search agent scaling. Moreover, verifier performance scales well with additional compute, with budget forcing and parallel sampling further improving its accuracy in filtering correct answers.


% These results point toward a compute-optimal paradigm for test-time scaling: rather than investing all budget into exploration, allocating a substantial share to verification yields higher returns. By balancing compute between search agents and verifiers—and applying sequential or parallel scaling where appropriate—we match the performance of leading closed-source Deep Research systems using only open-source models, with GLM-4.5, K2, and Qwen3 achieving * on BrowseComp, BrowseComp-ZH, Xbench-DeepSearch, and GAIA, respectively.

% These findings suggest a compute-optimal paradigm for test-time scaling. Rather than allocating all resources to exploration, dedicating a nontrivial share of compute to verification yields disproportionately higher gains. By systematically balancing compute across scaling targets (search agents versus verifiers), selecting scaling strategies suited to the task (sequential or parallel), and employing appropriate aggregation metrics, we demonstrate that open-source models such as GLM-4.5, K2, and Qwen3 can attain performance comparable to leading closed-source Deep Research systems across benchmarks including BrowseComp, BrowseComp-ZH, Xbench-DeepSearch, and GAIA.

% These findings point to a compute-optimal paradigm for test-time scaling. Instead of allocating all resources to exploration, dedicating a meaningful portion of compute to verification delivers disproportionately higher returns. By systematically balancing compute between search agents and verifier agents, choosing scaling strategies suited to the task (sequential or parallel), and applying the right aggregation metrics, we can upgrade open-source models such as GLM-4.5, K2, and Qwen3 into their ``Heavy'' variants through test-time scaling. 

These results highlight a compute-optimal paradigm for test-time scaling. Rather than allocating all resources to exploration, dedicating a substantial share of compute to verification yields disproportionately larger gains. By striking the right balance between search agents and verifier agents, selecting scaling strategies appropriate to the task (sequential or parallel), and applying effective aggregation metrics, we transform open-source models such as GLM-4.5, K2, Qwen3-2507 and Tongyi-DeepResearch into their ``Heavy'' variants through test-time scaling as exemplified in  Figure~\ref{fig:figure1} bottom right. In this way, open-source models achieve performance levels comparable to leading commercial systems as exemplified in Figure~\ref{fig:figure1} top part. Particularly, GLM-4.5 Heavy, an open-source system, performs on par with commercial leaders such as OpenAI DeepResearch and o3 across most benchmarks, achieving 54.0\% accuracy on BrowseComp, 49.0\% on BrowseComp-zh, 66.0\% on GAIA, and 68.0\% on xbench-DeepSearch. Tongyi-DeepResearch, designed for long-horizon information-seeking, further boosts performance, with the ``Heavy'' variant reaching 69\% accuracy on BrowseComp.

% \wz{I remove K2 and Qwen results, I think put too more results are not good}
%GLM-4.5 Heavy, K2 Heavy, and Qwen3-2507 Heavy reach accuracy of 54.0\%, 24.0\%, and 26.0\% on BrowseComp; 49.0\%, 36.0\%, and 42.0\% on BrowseComp-zh; 66.0\%, 58.3\%, and 53.4\% on GAIA; and 68.0\%, 57.0\%, and 63.0\% on xbench-DeepSearch. As an open-source system, GLM-4.5 Heavy performs on par with the best leading commercial choices such as OpenAI DeepResearch and o3 on most of these benchmarks. 
% GLM-4.5 Heavy, an open-source system, performs on par with commercial leaders such as OpenAI DeepResearch and o3 across most benchmarks, achieving 54.0\% accuracy on BrowseComp, 49.0\% on BrowseComp-zh, 66.0\% on GAIA, and 68.0\% on xbench-DeepSearch.




% In doing so, these deep research agents reach performance levels comparable to state-of-the-art closed-source Deep Research systems on benchmarks including BrowseComp, BrowseComp-ZH, XBench-DeepSearch, and GAIA.

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> scaling_both.tex <==
\section{Pushing Test-Time Scaling Limits of Open Models}
\label{sec:heavy_version}
% In this section, we integrate our previous findings to guide a balanced allocation of computation between search agents and verifier agents, as well as across different scaling strategies. We then evaluate how this allocation impacts performance across various models and benchmarks during further scaling.
% In this section, we extend our earlier findings to a wider set of benchmarks, examining how different allocations of computation—both between search agents and verifier agents, and across various scaling strategies—impact performance on these benchmarks.
% In this section, we \jhc{broaden our earlier findings to a wider range of benchmarks. To do this, we distribute computation between search agents and verifier agents, and apply various scaling strategies and aggregation metrics to construct the models' Heavy variants}{} as in Grok 4 Heavy~\citep{xai2025grok4}.




% \subsection{A Unified Framework for Scaling Test-Time Computation}
% \jh{this section is not necessary as a standalone section}
% Building on the results from \S~\ref{sec:scaling_searcher} and \S~\ref{sec:scaling_verifier}, we can conceptualize test-time compute scaling through three orthogonal dimensions: scaling target, scaling strategy, and aggregation metric.



% \begin{itemize}[leftmargin=*]
%     \item \textbf{Scaling target} defines what part of the system is being expanded—either the search agent, which explores candidate solutions, or the verifier agent, which evaluates and filters them.  
%     \item \textbf{Scaling strategy} specifies how the additional compute is applied, encompassing approaches such as Max \# Tool Call  (adjusting the maximum number of tool calls allowed), Budget Forcing (actively increasing tool invocation), and Parallel Scaling (running multiple trajectories concurrently).
%     \item \textbf{Aggregation metric} determines how the outputs are combined and assessed, using criteria like Pass@1 (single-best answer), Maj@K (majority voting), Weighted-of-K (confidence-weighted voting), or Best-of-K (selecting the highest-scoring candidate).\jh{it is not meaningful to include different maj@k and weighted-k in the last part of the experiments, because 1. they are not important and not practical, nobody really uses it in actual deployment; 2. they are making the figures confusing and too complex}
% \end{itemize}

%  This unified view helps disentangle where to allocate extra computation, how to deploy it, and how to measure its benefits—clarifying trade-offs and guiding compute-optimal scaling decisions.

\begin{table*}[t]
\centering
\caption{Accuracy (\%) of proprietary and open-source agentic systems across multiple benchmarks. Results marked with \textdagger{} are from our test runs, indicating the maximum Pass@1 that models can achieve when provided with sufficient tool calls without budget forcing. For Tongyi DeepResearch, we report both the results of our test runs and the officially reported results}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
                    & \textbf{BrowseComp}  & \textbf{BrowseComp-zh} & \textbf{GAIA} & \textbf{xbench-DeepSearch} \\
\midrule
\multicolumn{5}{c}{Proprietary Deep-Research Systems / Models} \\
\midrule
Gemini 2.5 Pro & 7.6 & 27.3 & - & - \\
OpenAI o1 & 9.9 & 29.1 & - & - \\
OpenAI o3\textsuperscript{\textdagger}         & 55.0  & 59.0 & 68.0 & 68.0 \\
OpenAI GPT-5 & 19.8 & 34.3 & - & 30.0 \\
Grok3 DeepResearch  &       & 12.9 & -    & 50+ \\
Doubao DeepResearch & -     & 26.0 & -    & 50+ \\
OpenAI DeepResearch & 51.5 & 42.9 & 70.5 & 66.7 \\
\midrule
\multicolumn{5}{c}{Open-Source Models} \\
\midrule
DeepSeek-R1 & 2.0 & 23.2 & 16.5 & 32.7 \\
Qwen3-2507\textsuperscript{\textdagger}          & 8.0  & 23.0 & 44.7 & 45.5 \\
K2\textsuperscript{\textdagger}                 & 11.0 & 22.0 & 50.0 & 54.0 \\
GLM-4.5\textsuperscript{\textdagger}             & 19.0 & 27.0 & 58.0 & 58.0 \\
DeepSeek-V3.1 & 30.0 & 49.2 & - & 71.2 \\
Tongyi DeepResearch\textsuperscript{\textdagger} & 43.0 & 39.0 & 70.6 & 68.0 \\
Tongyi DeepResearch & 43.4 & 46.7 & 70.9 & 75.0 \\
\midrule
\multicolumn{5}{c}{Open-Source Models (Heavy Version)} \\
\midrule
\rowcolor{gray!12} Qwen3-2507 Heavy
& \textbf{29.0} \textcolor{green!50!black}{(+21.0)}
& \textbf{42.0} \textcolor{green!50!black}{(+19.0)}
& \textbf{53.4} \textcolor{green!50!black}{(+8.7)}
& \textbf{63.0} \textcolor{green!50!black}{(+17.5)} \\
\rowcolor{gray!12} K2 Heavy
& \textbf{24.0} \textcolor{green!50!black}{(+13.0)}
& \textbf{36.0} \textcolor{green!50!black}{(+14.0)}
& \textbf{58.3} \textcolor{green!50!black}{(+8.3)}
& \textbf{57.0} \textcolor{green!50!black}{(+3.0)} \\
\rowcolor{gray!12} GLM-4.5 Heavy
& \textbf{54.0} \textcolor{green!50!black}{(+35.0)}
& \textbf{49.0} \textcolor{green!50!black}{(+22.0)}
& \textbf{66.0} \textcolor{green!50!black}{(+8.0)}
& \textbf{68.0} \textcolor{green!50!black}{(+10.0)} \\
\rowcolor{gray!12} Tongyi DeepResearch Heavy
& \textbf{69.0} \textcolor{green!50!black}{(+26.0)}
& \textbf{55.0} \textcolor{green!50!black}{(+16.0)}
& \textbf{72.8} \textcolor{green!50!black}{(+2.2)}
& \textbf{80.0} \textcolor{green!50!black}{(+12.0)} \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
% \caption{Accuracy (\%) of proprietary and open-source agentic systems across multiple benchmarks. Results marked with \textdagger{} are from our test runs, indicating the maximum Pass@1 that models can achieve when provided with sufficient tool calls without budget forcing. For Tongyi DeepResearch, we report both the results of our test runs and the officially reported results}
\label{table:result_with_tts}
\vspace{-15pt}
\end{table*}

\subsection{Experimental Setup}

% \paragraph{A Unified View for Scaling Test-Time Computation} 
Building on the results from \S\ref{sec:scaling_searcher} and \S\ref{sec:scaling_verifier}, we can conceptualize test-time compute scaling through three orthogonal dimensions: scaling target, scaling strategy, and aggregation metric. \textbf{Scaling target} defines what part of the system is being expanded—either the search agent, which explores candidate solutions, or the verifier agent, which evaluates and filters them.  
\textbf{Scaling strategy} specifies how the additional compute is applied, encompassing approaches such as Max \# Tool Call  (adjusting the maximum number of tool calls allowed), Budget Forcing (actively increasing tool invocation), and Parallel Scaling (running multiple trajectories concurrently).
\textbf{Aggregation metric} determines how the outputs are combined and assessed, using criteria like Pass@1 (single-best answer), Maj@K (majority voting), Weighted Voting (confidence-weighted voting), or Best-of-K (selecting the highest-scoring candidate). This unified view helps disentangle where to allocate extra computation, how to deploy it, and how to measure its benefits, clarifying trade-offs and guiding compute-optimal scaling decisions. 
% \wz{I'm keeping the definitions of maj@k, best-of-k, and weighted voting there, but removing maj@k and weighted voting from the figure and experiment analysis. And put the detail of the metric used in Appendix}

\paragraph{Benchmarks and Models}
Compared to evaluating the agent on QA tasks that are relatively simple, we aim to assess its information-seeking capabilities using significantly more challenging benchmarks. Specifically, we evaluate on the following benchmarks: (1) BrowseComp~\citep{wei2025browsecomp}, which includes complex search problems that require navigating through a large space of potential answers, where relevant information is difficult to locate. (2) BrowseComp-zh~\citep{zhou2025browsecomp}, the Chinese counterpart of BrowseComp to evaluate LLM agents on the Chinese web. (3) GAIA~\citep{mialon2023gaia}, which evaluates multi-modality and tool-use capabilities; following previous work~\citep{li2025websailor}, we focus on its text-only validation set. (4) xbench-DeepSearch~\citep{chen2025xbench}, another challenging benchmark designed to assess tool usage capabilities specifically in search and information retrieval contexts. The models used remain consistent with those in \S\ref{sec:scaling_searcher} and \S\ref{sec:scaling_verifier}. We also include Tongyi-DeepResearch-30B-A3B~\citep{tongyidr}, a model that is specifically designed for long-horizon, deep information-seeking tasks. Our evaluation uses 100 randomly sampled tasks from BrowseComp and BrowseComp-zh, since running the full test is computationally expensive. This sampling balances cost efficiency with representativeness. In contrast, evaluations for other benchmarks are conducted on their full datasets.

\paragraph{Scaling Details} 

We scale performance by combining Max \# Tool Call scaling with Budget Forcing to reach the Pass@1 peaks of different models. To broaden the exploration space of the search agents, we apply parallel scaling on top of sequential scaling. For example, on BrowseComp, GLM-4.5 generates 32 parallel samples, K2 generates 24, and Qwen3-2507 generates 16, while on other benchmarks every model samples  8 times in parallel. Once these trajectories are produced, a verifier selects the answers, after which parallel scaling or budget forcing is applied again to the verifier to increase the verifier’s test-time compute. 
These scaling approaches lead to the heavey variant of different models.
We document the specific scaling setup for GLM-4.5 Heavy, K2 Heavy, and Qwen3-2507 Heavy in Appendix~\ref{sec:scaling_details_heavy_variant}. 


% Building on the findings from Section ~\ref{sec:scaling_searcher} and ~\ref{sec:scaling_verifier}, we can view test-time computation scaling through a unified framework with three orthogonal dimensions: \textbf{scaling target}, \textbf{scaling strategy}, and \textbf{aggregation metric}. The scaling target specifies which system component is being scaled—either the search agent or the verifier agent. The scaling strategy defines the method of scaling, such as Max \# Tool Call, Budget Forcing, or Parallel Scaling. The aggregation metric determines how the final answers are combined and evaluated, using measures such as Pass@1, Maj@K, Weighted-of-K, or Best-of-K.


\subsection{Experimental Results}
% \begin{table*}[t]
% \centering
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{lcccc}
% \hline
%                        & \textbf{BrowseComp}  & \textbf{BrowseComp-zh} & \textbf{GAIA} & \textbf{xbench-DeepSearch} \\ \hline
% \multicolumn{5}{c}{Proprietary Deep-Research Systems}                                                    \\ \hline
% OpenAI DeepResearch/o3 & 51.5                 & 42.9                   & 70.5          & 66.7                       \\
% Grok3 DeepResearch     & \multicolumn{1}{l}{} & 12.9                   & -             & 50+                        \\
% Doubao DeepResearch    & -                    & 26.0                   & -             & 50+                        \\ \hline
% \multicolumn{5}{c}{Open-Source Models — Search Agent Only}                                              \\ \hline
% Qwen3-2507             & 18.0                 & 30.0                   & 49.5          & -                          \\
% K 2                    & 14.0                 & 22.0                   & 51.5          & -                          \\
% GLM 4.5                & 27.0                 & 33.0                   & 58.3          & -                          \\ \hline
% \multicolumn{5}{c}{Open-Source Models — Search + Verifier Agents}                                         \\ \hline
% Qwen3-2507             & 26.0 (+8.0)          & 49.0 (+19.0)           & 53.4 (+3.9)   & -                          \\
% K 2                    & 24.0 (+10.0)         & 36.0 (+14.0)           & 58.3 (+6.8)   & -                          \\
% GLM 4.5                & 47.0 (+20.0)         & 49.0 (+16.0)           & 66.0 (+7.7)   & -                          \\ \hline
% \end{tabular}
% }
% \caption{Pass@1 and the average number of actual tool uses per problem for models, under a maximum limit of 15 search tool calls. Note that ``Qwen3-2507'' refers to Qwen3-235B-A22B-Instruct-2507. For the BrowseComp-en and BrowseComp-zh benchmarks, results are based on 100 randomly sampled problems, while the full problem sets are used for the other benchmarks.}
% \label{table:result_wo_tts}
% % \vspace{-12pt}
% \end{table*}

% \begin{table*}[t]
% \centering
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
%  & \textbf{BrowseComp} & \textbf{BrowseComp-zh} & \textbf{GAIA} & \textbf{XBench-DeepSearch} \\
% \midrule
% \multicolumn{5}{c}{\textbf{Proprietary Deep-Research Systems}} \\
% \midrule
% OpenAI DeepResearch / o3 & 51.5 & 42.9 & 70.5 & 66.7 \\
% Grok3 DeepResearch        & --   & 12.9 & --   & 50+  \\
% Doubao DeepResearch       & --   & 26.0 & --   & 50+  \\
% \midrule
% \multicolumn{5}{c}{\textbf{Open-Source Models — Search Agent Only}} \\
% \midrule
% Qwen3-2507 & 18.0 & 30.0 & 49.5 & -- \\
% K2         & 14.0 & 22.0 & 51.5 & -- \\
% GLM-4.5    & 27.0 & 33.0 & 58.3 & -- \\
% \midrule
% \multicolumn{5}{c}{\textbf{Open-Source Models — Search + Verifier Agents}} \\
% \midrule
% Qwen3-2507 & 26.0 \textcolor{gray}{(+8.0)}  & 49.0 \textcolor{gray}{(+19.0)} & 53.4 \textcolor{gray}{(+3.9)} & -- \\
% K2         & 24.0 \textcolor{gray}{(+10.0)} & 36.0 \textcolor{gray}{(+14.0)} & 58.3 \textcolor{gray}{(+6.8)} & -- \\
% GLM-4.5    & 47.0 \textcolor{gray}{(+20.0)} & 49.0 \textcolor{gray}{(+16.0)} & 66.0 \textcolor{gray}{(+7.7)} & -- \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different agentic systems across different benchmarks}
% \label{table:result_with_tts}
% \end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
%  & \textbf{BrowseComp} & \textbf{BrowseComp-zh} & \textbf{GAIA} & \textbf{XBench-DeepSearch} \\
% \midrule
% \multicolumn{5}{c}{\textbf{Proprietary Deep-Research Systems}} \\
% \midrule
% OpenAI DeepResearch / o3 & 51.5 & 42.9 & 70.5 & 66.7 \\
% Grok3 DeepResearch        & --   & 12.9 & --   & 50+  \\
% Doubao DeepResearch       & --   & 26.0 & --   & 50+  \\
% \midrule
% \multicolumn{5}{c}{\textbf{Open-Source Models — Search Agent Only}} \\
% \midrule
% Qwen3-2507 (single attempt) & 18.0 & 30.0 & 49.5 & 58.0 \\
% K2 (single attempt)         & 14.0 & 22.0 & 51.5 & 54.0 \\
% GLM-4.5 (single attempt)    & 27.0 & 33.0 & 58.3 & 58.0 \\
% Qwen3-2507 (multiple attempts) & 21.0 & 32.7 & 50.0 & 63.0   \\
% K2 ((multiple attempts)         & 15.3 & 29.2 & 52.5 & 57.0   \\
% GLM-4.5 ((multiple attempts)    & 40.6 & 39.8 & 59.8 & 68.0   \\
% \midrule
% \multicolumn{5}{c}{\textbf{Open-Source Models — Search + Verifier Agents}} \\
% \midrule
% Qwen3-2507 (multiple attempts) & 26.0 & 49.0 & 53.4 & -- \\
% K2 (multiple attempts)         & 24.0 & 36.0 & 58.3 & -- \\
% GLM-4.5 (multiple attempts)    & 47.0 & 49.0 & 66.0 & -- \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of proprietary and open-source agentic systems across multiple benchmarks. ``Single attempt'' settings allow no majority voting or parallel test-time compute; ``multiple attempts'' settings allow test-time selection of the candidate answer.  For open-source models, we report results from two settings: (1) scaling only the search agent’s test-time compute—showing both Pass@1 and majority-vote accuracy; and (2) scaling both the search and verifier agents—reporting the best verifier-based voting result (best-of-n or weighted-of-n). For BrowseComp-en, majority voting uses n = 16 and the verifier result is the higher of best-of-16 or weighted-of-16. For all other benchmarks, majority voting uses n = 8 and the verifier result is the higher of best-of-8 or weighted-of-8.}
% \label{table:result_with_tts}
% \end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
%  & \textbf{Attempt} & \textbf{BrowseComp} & \textbf{BrowseComp-zh} & \textbf{GAIA} & \textbf{XBench-DeepSearch} \\
% \midrule
% \multicolumn{6}{c}{\textbf{Proprietary Deep-Research Systems}} \\
% \midrule
% OpenAI DeepResearch / o3 & -- & 51.5 & 42.9 & 70.5 & 66.7 \\
% Grok3 DeepResearch        & -- & --   & 12.9 & --   & 50+  \\
% Doubao DeepResearch       & -- & --   & 26.0 & --   & 50+  \\
% \midrule
% \multicolumn{6}{c}{\textbf{Open-Source Models — Search Agent Only}} \\
% \midrule
% \multirow{2}{*}{Qwen3-2507} & Single   & 18.0 & 30.0 & 49.5 & 58.0 \\
%                             & Multiple & 21.0 & 32.7 & 50.0 & 63.0 \\
% \multirow{2}{*}{K2}         & Single   & 14.0 & 22.0 & 51.5 & 54.0 \\
%                             & Multiple & 15.3 & 29.2 & 52.5 & 57.0 \\
% \multirow{2}{*}{GLM-4.5}    & Single   & 27.0 & 33.0 & 58.3 & 58.0 \\
%                             & Multiple & 40.6 & 39.8 & 59.8 & 68.0 \\
% \midrule
% \multicolumn{6}{c}{\textbf{Open-Source Models — Search + Verifier Agents}} \\
% \midrule
% \multirow{1}{*}{Qwen3-2507} & Multiple & 26.0 & 42.0 & 53.4 & -- \\
% \multirow{1}{*}{K2}         & Multiple & 24.0 & 36.0 & 58.3 & -- \\
% \multirow{1}{*}{GLM-4.5}    & Multiple & 47.0 & 49.0 & 66.0 & -- \\
% \bottomrule
% \end{tabular}
% }
% \caption{\jh{this table needs to be re-organized }Performance comparison of proprietary and open-source agentic systems across multiple benchmarks. ``Single attempt'' settings allow no majority voting or parallel test-time compute; ``multiple attempts'' settings allow test-time selection of the candidate answer.  For open-source models, we report results from two settings: (1) scaling only the search agent’s test-time compute—showing both Pass@1 and majority-vote accuracy; and (2) scaling both the search and verifier agents—reporting the best verifier-based voting result (best-of-n or weighted-of-n). For BrowseComp-en, majority voting uses n = 16 and the verifier result is the higher of best-of-16 or weighted-of-16. For all other benchmarks, majority voting uses n = 8 and the verifier result is the higher of best-of-8 or weighted-of-8.}
% \label{table:result_with_tts}
% \end{table*}
\begin{figure}[!t]
        \centering
\includegraphics[width=0.99\columnwidth]{iclr2026/fig/Figure_1_browse.pdf}
\vspace{-10pt}
\caption{Scaling test time compute for different models on BrowseComp, where the x-axis represents the actual number of tool calls, and the y-axis represents accuracy.}
        \label{fig:browse_experiment_results_comparisonv2}
\vspace{-15pt}
\end{figure}


Table~\ref{table:result_with_tts} presents the experimental results of GLM-4.5 Heavy, K2 Heavy, and Qwen3-2507 Heavy. The three models after test-time scaling achieve substantial performance gains across all benchmarks. For example, Qwen3-2507 Heavy improves accuracy over Qwen3-2507 by about 20 absolute points on BrowseComp, BrowseComp-zh, and xbench-DeepSearch. Notably, GLM-4.5 Heavy reaches 54.0\% accuracy on BrowseComp, 66.0\% on GAIA, and 68.0\% on xbench-DeepSearch, putting it on par with the best commercial agents such as o3 and OpenAI Deep Research on these three benchmarks. We also introduce a heavy variant of Tongyi Deep Research, which achieves 69\% accuracy on BrowseComp, 55\% accuracy on BrowseComp-zh, 72.8\% on GAIA and 80.0\% on xbench-DeepSearch as shown in Figure~\ref{fig:figure1}. Full implementation details are provided in the Appendix~\ref{sec:scaling_details_heavy_variant}. 


Figure~\ref{fig:browse_experiment_results_comparisonv2} presents the results of scaling test-time compute for different models on BrowseComp. Sustained compute expansion can bring open-source systems close to closed-source performance. Verifier introduction further accelerates performance gains. For K2, adding a verifier increases Best-of-16 to 23\%, with a slope much steeper than simply expanding the search agent. Figure~\ref{fig:browse-zh_experiment_results_comparisonv2} in Appendix~\ref{sec:scaling_browsecomp_zh} shows that performance patterns on BrowseComp-zh closely mirror those on BrowseComp. On BrowseComp-zh, GLM-4.5 attains a Best-of-8 score of 49\%, exceeding the level of OpenAI Deep Research (see Table \ref{table:result_with_tts}). Notably, parallel scaling of the verifier yields consistent accuracy gains: for K2, Best-of-8 rises from 31\% to 36\%. This is because parallel sampling mitigates variance in individual confidence scores, making the selection process more robust to noise by reducing the impact of extreme values. Figure~\ref{fig:gaia_experiment_results_comparisonv2} in Appendix ~\ref{sec:scaling_gaia} presents the results of scaling test-time compute for different models on GAIA. Across models, different scaling strategies still yield notable performance gains for both search agents and verifier agents. We report xbench-DeepSearch results in Figure~\ref{fig:xbench_experiment_results_comparisonv1} of the Appendix. Because solving and verifying tasks in this benchmark are nearly equally difficult (as detailed in Appendix~\ref{sec:scaling_xbench}), we only evaluate search-agent scaling in Figure~\ref{fig:xbench_experiment_results_comparisonv1} and Table~\ref{table:result_with_tts}.

%However, further parallel scaling of the verifier yields diminishing returns, rising only from 23\% to 24\%, highlighting the need for coordinated scaling of both search and verifier agents to sustain growth.


% \begin{figure}[!t]
%         \centering
% \includegraphics[width=0.99\columnwidth]{iclr2026/fig/Figure_2_browsecomp-zh.pdf}
% \vspace{-10pt}
% \caption{Scaling test time compute for different models on Browsecomp-zh, where the x-axis represents the actual number of tool calls, and the y-axis represents accuracy.}
%         \label{fig:browse-zh_experiment_results_comparisonv2}
%         \vspace{-10pt}
% \end{figure}

% Figure~\ref{fig:browse-zh_experiment_results_comparisonv2} shows that performance patterns on BrowseComp-zh closely mirror those on BrowseComp. On BrowseComp-zh, GLM-4.5 attains a Best-of-8 score of 49\%, exceeding the level of OpenAI Deep Research (see Table \ref{table:result_with_tts}). Notably, parallel scaling of the verifier yields consistent accuracy gains: for K2, Best-of-8 rises from 31\% to 36\%. This is because parallel sampling mitigates variance in individual confidence scores, making the selection process more robust to noise by reducing the impact of extreme values.

% \begin{figure}[!t]
%         \centering
% \includegraphics[width=0.99\columnwidth]{iclr2026/fig/Figure_3_gaia.pdf}
% \vspace{-10pt}
% \caption{Scaling test time compute for different models on GAIA, where the x-axis represents the actual number of tool calls, and the y-axis represents accuracy.}
%         \label{fig:gaia_experiment_results_comparisonv2}
%         \vspace{-10pt}
% \end{figure}

% Figure~\ref{fig:gaia_experiment_results_comparisonv2} presents the results of scaling test-time compute for different models on GAIA. Across models, different scaling strategies still yield notable performance gains for both search agents and verifier agents. For instance, Budget Forcing improves Qwen3-2507’s search agent accuracy from 44\% to 50\%, while Parallel Scaling raises K2’s verifier weighted voting score from 54\% to 58\%. However, unlike in BrowseComp and BrowseComp-zh, scaling verifier compute offers a smaller efficiency advantage on GAIA. This is because GAIA poses lower information-retrieval difficulty: as shown in Figures~\ref{fig:browse_experiment_results_comparisonv2} and~\ref{fig:browse-zh_experiment_results_comparisonv2}, BrowseComp requires over five times more tool calls than GAIA. With this smaller search burden, the gap between solving a task and verifying its correctness narrows, reducing the relative benefit of the verifier agent. We report xbench-DeepSearch results in Figure~\ref{fig:xbench_experiment_results_comparisonv1} of the Appendix. Because solving and verifying tasks in this benchmark are nearly equally difficult (as detailed in Appendix~\ref{sec:scaling_xbench}), we only evaluate search-agent scaling in Figure~\ref{fig:xbench_experiment_results_comparisonv1} and Table~\ref{table:result_with_tts}.

==> scaling_policy.tex <==
\section{Scaling Search Compute}
\label{sec:scaling_searcher}
In this section, we begin by presenting the framework of the search agent and methods for scaling compute. We then outline the experimental setup, specifying the benchmarks, models, and evaluation metrics employed. Lastly, we report the experimental results on scaling the search agent's test-time compute within the proposed framework.

\subsection{Overview of the Search Agent Framework}
\label{sec:search_agent_framework}
To ensure scalability and generality, we design a streamlined framework based on ReAct~\citep{yao2023react}. In this framework, the search agent handles user problems by iteratively reasoning, generating and executing actions, and processing observations received from real-world web environments. The agent's action space includes either generating a final answer or invoking search tools. The search tool itself combines the web search and browsing functionalities introduced in WebThinker~\citep{li2025webthinker}: it takes as input a search query and an explicit search intent, and returns organized information retrieved from the web. Within this tool, an auxiliary model determines how to organize retrieved content or whether additional browsing is needed. To study test-time compute scaling in a controlled setting, we select K2 as the auxiliary model across the entire paper and do not change it (see Appendix~\ref{sec:impact_aux} for details on this choice). Similar frameworks with searching and browsing functionalities based on ReAct have been widely adopted to develop web searching agents~\citep{li2025websailor,liu2025webexplorer,gao2025beyond}.
% \wz{add the explanation in this paragraph, plz check}

% To enable the agent to focus on high-level planning and tool use, we encapsulate a flexible search tool inspired by WebThinker~\citep{li2025webthinker}. This tool accepts a search query and search intent as inputs, and returns organized information in response. Internally, the tool uses a search engine to retrieve and navigate relevant webpages, while an auxiliary language model extracts relevant information according to the search intent. This auxiliary model also autonomously decides whether to issue follow-up queries or click on urls within webpages to continue the information extraction process. \jh{this sounds complex, isn't this just a normal search tool + a browsing tool? The current descriptions seems to regard browsing as part of the ``flexible search tool'', this is not a common way of viewing it nowadays. If the browsing tool is directly taken from WebThinker then we just say it. We don't want our scaffold sound fancy or complex as it is not our goal, instead, it is better that we can clarify the relations between our scaffold and other works like WebThinker, Websailor, and it is the best to emphasize that we use a simple scaffold similar to previous works. We don't want others to see our gains from some special scaffold or better scaffold than previous works}

%To manage computational cost, we define a maximum number of allowed tool calls in the search agent's system prompt. Once this limit is reached, the agent receives no further results from the search tool. The system prompt used for the agent is provided in Appendix. (mentioned it in method)

\subsection{Test-Time Scaling Approaches}
We categorize methods for scaling the search agent's compute into two types:  

\paragraph{Sequential Scaling} increases computational resources along a single agentic trajectory for each individual problem. We introduce two straightforward yet effective methods: (1) \emph{Max \# Tool Call}: It is common practice to establish a maximum number of tool calls allowed for the search agent, which is explicitly defined in the agent's system prompt. Once the agent reaches this limit, no additional results are provided from the search tool. We experiment with this approach to encourage more tool callings, and details of the system prompt configuration are available in Figure~\ref{fig:searcher-prompt}. (2) \emph{Budget Forcing}: Our experiments revealed that agents often terminate tasks prematurely, even when the system prompt permits sufficient tool calls. Inspired by the approach in~\citet{muennighoff2025s1}, after the agent produces an initial final answer, we allocate additional budget for further tool usage and instruct the agent to continue exploring alternative solution paths or search strategies. Examples of budget forcing scenarios can be found in the Figure~\ref{fig:budget_forcing_example}.
% \paragraph{Parallel Scaling} increases computation by sampling multiple independent trajectories simultaneously for the same problem. We independently sample multiple trajectories for each problem and determine the final answer by applying majority voting to these predicted answers.\jh{here we need to introduce verify-and-select together with majority voting. Just as in sequential scaling, here can be done with two bullet points, while we can say we will present results for majority voting first, and in xxx we will discuss verification. Also, it is important to note that majority voting is not really a practical approach here as it cannot be directly applied for open generation.}

\paragraph{Parallel Scaling} expands computation by generating multiple independent solution trajectories for the same problem in parallel and then applying aggregation methods to determine the final output. We classify these aggregation methods into two types, depending on whether they rely on an external verifier: (1) \emph{Majority Voting}: This approach follows the self-consistency principle~\citep{wang2022self}, where the model independently produces multiple trajectories, and the most frequently predicted answer is selected as the final output. However, majority voting has limited practicality, as it cannot easily extend to open-ended generation tasks where answers are diverse and not strictly comparable. (2) \emph{Verifier-Based}: These approaches employ an external verifier to assign scores to the sampled trajectories. Based on these scores, one can either adopt \emph{Best-of-K}, which selects the trajectory with the highest score, or \emph{Weighted Voting}, which aggregates candidate trajectories by weighting them according to their verifier-assigned scores. In what follows, we first report results obtained using \emph{Majority Voting} where we focus on analyzing the search agent alone, while in \textsection\ref{sec:scaling_verifier} we present experiments incorporating verifier-based strategies.

\begin{figure}[t]
\vspace{-10pt}
        \centering
\includegraphics[width=0.98\textwidth]{iclr2026/fig/policy_model_performance_vs_compute_seq_sep_v8.pdf}
\vspace{-10pt}
\caption{Sequential scaling of compute, with the x-axis representing the actual number of tool calls, and the y-axis representing Pass@1 accuracy on BrowseComp. For Max \# Tool Call, search tool limits are set to 15, 30, and 50 for Qwen3-2507 and K2, and 15, 30, 50, and 100 for GLM-4.5. Budget Forcing begins from each model’s peak Max \# Tool Call setting and expands until saturation: Qwen3-2507 starts at 15, adding 15 tools per step (7 expansions); K2 starts at 30, adding 30 per step (2 expansions); GLM-4.5 starts at 50, adding 50 per step (2 expansions).
        }
        \label{fig:scaling_policy_seq}
    \vspace{-15pt}

\end{figure}


% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_baseline_bar.pdf}\vspace{-10pt}
%     \caption{Pass@1 and the average number of actual tool uses per problem for models, under a maximum limit of 15 search tool calls. Note that ``Qwen3-2507'' refers to Qwen3-235B-A22B-Instruct-2507.\wz{todo: Change all accuracy values in figures from decimals to percentages}}
%     \label{fig:result_wo_tts}
%     % \vspace{-10pt}
% \end{wrapfigure}

\subsection{Experimental Setup}
\label{sec:scaling_search_setup}
\paragraph{Benchmarks and Models}
% Compared to evaluating the agent on QA tasks that are relatively simple, we aim to assess its information-seeking capabilities using significantly more challenging benchmarks. Specifically, we evaluate on the following benchmarks: (1) BrowseComp-en~\citep{wei2025browsecomp}, which includes complex search problems that require navigating through a large space of potential answers, where relevant information is difficult to locate. (2) BrowseComp-zh~\citep{zhou2025browsecomp}, the Chinese counterpart of BrowseComp-en. (3) GAIA~\citep{mialon2023gaia}, which evaluates multi-modality and tool-use capabilities; following previous work~\citep{li2025websailor}, we focus on its text-only validation set. (4) XbenchDeepSearch~\citep{chen2025xbench}, another challenging benchmark designed to assess tool usage capabilities specifically in search and information retrieval contexts.
% \paragraph{Models} We select three open-source models with strong reasoning and agentic capabilities, GLM-4.5\footnote{\url{https://z.ai/blog/glm-4.5}}, K2~\citep{team2025kimi}, and Qwen3-235B-A22B-Instruct-2507~\citep{yang2025qwen3}, as search agents to evaluate their effectiveness when scaling test-time compute. Additionally, we choose K2 as the auxiliary model for the search tool (A detailed analysis of our choice of auxiliary model is provided in the Appendix~\ref{}).


To rigorously evaluate the agent’s information-seeking capabilities, we use benchmarks that are substantially more challenging than standard QA tasks. For this section and \S\ref{sec:scaling_verifier}, we use BrowseComp~\citep{wei2025browsecomp} to study test-time scaling in a series of controlled experiments, where the search queries are complex and require navigation through a vast space of potential answers. Since the complete BrowseComp includes about 1200 questions, completing the full test consumes substantial computational resources. Therefore, a random sample of 100 is used to reduce costs while still being representative enough to reflect performance on the full dataset. In \S\ref{sec:heavy_version}, we will include more benchmarks to present the final test-time scaling results. We select three open-source models with strong reasoning and agentic capabilities, GLM-4.5~\citep{zeng2025glm}, K2~\citep{team2025kimi}, and Qwen3-235B-A22B-Instruct-2507~\citep{yang2025qwen3}, as search agents to evaluate their effectiveness when scaling test-time compute.

\paragraph{Metrics}
% To comprehensively measure the test-time compute requirements of search agents for each problem, we use the following metrics: \jh{in these figures we never use FLOPs right?}\textbf{inference FLOPs} (including FLOPs from both the search agent itself and the auxiliary model \jhc{}{such as xxx}), the total number of \textbf{interaction turns}, and the actual number of \textbf{tool calls} made\jh{what is the difference between interaction turns and tool calls? Please clarify, and why do we need both}. 
% We measure the test-time compute of search agents by the actual number of \textbf{tool calls} they make to solve each problem. 
Following prior work~\citep{gao2025beyond,li2025websailor}, we approximate the test-time compute of search agents by counting the actual number of tool calls they make to solve each problem. This choice reflects the nature of deep research tasks, which often require interacting with external tools to gather information. 
% In contrast, relying solely on a model’s internal knowledge and producing more reasoning tokens typically makes it harder to arrive at correct answers. 
% We compare test-time scaling statistics using both tokens and tool calls in Table~\ref{table:diff_metric} in the Appendix\jh{let's remove table 3, not very meaningful, tokens between different models are not that comparable. Apparently if comparing compute across models, the number of tool calls is not a good approximator for compute, but we believe it is a good approximator when comparing compute of the same model while scaling up}. The results show that GLM 4.5\jh{GLM-4.5, be consistent} achieves a significantly higher Pass@1 than Qwen3. Notably, this improvement does not come with a substantial increase in output tokens, but it is accompanied by more than twice the number of tool calls compared to Qwen3\jh{remove this if removing table 3}.
To evaluate the performance of the search agent, we use two metrics: \textbf{Pass@K}, which measures whether the search agent finds the correct answer at least once among K independently sampled trajectories; and \textbf{Maj@K}, which measures whether the correct answer matches the majority vote among the answers from K independently sampled trajectories. 
\subsection{Experimental Results}

% \begin{table*}[t]
% \centering
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{lcccccccc}
% \hline
%            & \multicolumn{2}{c}{\textbf{BrowseComp-en}} & \multicolumn{2}{c}{\textbf{BrowseComp-zh}} & \multicolumn{2}{c}{\textbf{GAIA}}    & \multicolumn{2}{c}{\textbf{XbenchDeepSearch}} \\
%            & \textbf{Pass@1}    & \textbf{Tool Call}    & \textbf{Pass@1}    & \textbf{Tool Call}    & \textbf{Pass@1} & \textbf{Tool Call} & \textbf{Pass@1}      & \textbf{Tool Call}     \\ \hline
% Qwen3-2507 & 0.08               & 9.0                   & 0.15               & 5.1                   & 0.45            & 3.1                & 0.45                 & 3.2                    \\
% K2         & 0.04               & 11.6                  & 0.22               & 5.6                   & 0.47            & 3.5                & 0.46                 & 3.3                    \\
% GLM 4.5    & 0.10               & 15.0                  & 0.22               & 12.4                  & 0.52            & 6.0                & 0.58                 & 6.1                    \\ \hline
% \end{tabular}
% }
% \caption{Pass@1 and the average number of actual tool uses per problem for models, under a maximum limit of 15 search tool calls. Note that ``Qwen3-2507'' refers to Qwen3-235B-A22B-Instruct-2507. For the BrowseComp-en and BrowseComp-zh benchmarks, results are based on 100 randomly sampled problems, while the full problem sets are used for the other benchmarks.}
% \label{table:result_wo_tts}
% % \vspace{-12pt}
% \end{table*}


% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_baseline_bar.pdf}\vspace{-10pt}
%     \caption{Pass@1 and the average number of actual tool uses per problem for models, under a maximum limit of 15 search tool calls. Note that ``Qwen3-2507'' refers to Qwen3-235B-A22B-Instruct-2507. For the BrowseComp-en, results are based on 100 randomly sampled problems.}
%     \label{fig:result_wo_tts}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \paragraph{Models falter on challenging problems without enough search tool usage. } We cap tool usage at 15 and evaluate various models on BrowseComp-en. As shown in Figure~\ref{fig:result_wo_tts}, overall performance is mediocre on  BrowseComp-en, where no open-source model surpasses 10\% accuracy, while OpenAI's DeepResearch system could reach 50\%. The results also show that models typically use up all available tool calls on harder benchmarks. For instance, GLM 4.5 averages 15 tool uses on BrowseComp-en, suggesting that higher tool quotas are needed for better performance.\jh{this experiment and paragraph does not seem very useful. I think tool conditional performance scaling already conveys the message of this paragraph}



% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_baseline_bar.pdf}\vspace{-10pt}
%     \caption{Pass@1 and the average number of actual tool uses per problem for models, under a maximum limit of 15 search tool calls. Note that ``Qwen3-2507'' refers to Qwen3-235B-A22B-Instruct-2507. For the BrowseComp-en, results are based on 100 randomly sampled problems.}
%     \label{fig:result_wo_tts}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \begin{figure}[t]
%     \centering
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \resizebox{\textwidth}{!}{
%             \includegraphics{iclr2026/fig/policy_model_performance_vs_compute_seqv10.pdf}
%         }
%         \vspace{-10pt}
%         \caption{\jh{from the legend we cannot tell the dashed lines are budgetforcing, should make it more clear in the figure itself besides the caption (similar for other figures, plz revise)}Sequential scaling of compute, with the x-axis representing the actual number of tool calls, and the y-axis representing pass@1. For Tool Conditional(solid lines), search tool limits were set to 15, 30, and 50 for Qwen3-2507 and K2, and 15, 30, 50, and 100 for GLM 4.5. Budget Forcing(dashed lines) begins from each model’s peak Tool Conditional setting and expands until saturation: Qwen3-2507 starts at 15, adding 15 tools per step (7 expansions); K2 starts at 30, adding 30 per step (2 expansions); GLM 4.5 starts at 50, adding 50 per step (2 expansions).} 
%         \label{fig:scaling_policy_seq}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \resizebox{\textwidth}{!}{
%             \includegraphics{iclr2026/fig/policy_model_performance_metrics_palv5.pdf}
%         }
%         \vspace{-10pt}
%         \caption{Sequential scaling of compute, with the x-axis representing the actual number of tool calls, and the y-axis representing pass@1. For Tool Conditional(solid lines), search tool limits were set to 15, 30, and 50 for Qwen3-2507 and K2, and 15, 30, 50, and 100 for GLM 4.5. Budget Forcing(dashed lines) begins from each model’s peak Tool Conditional setting and expands until saturation: Qwen3-2507 starts at 15, adding 15 tools per step (7 expansions); K2 starts at 30, adding 30 per step (2 expansions); GLM 4.5 starts at 50, adding 50 per step (2 expansions).}
%         \label{fig:scaling_policy_pal}
%     \end{minipage}
%     \vspace{-15pt}
% \end{figure}





% \begin{figure}[t]
% \vspace{-10pt}
%         \centering
% \includegraphics[width=0.98\textwidth]{iclr2026/fig/policy_model_performance_metrics_pal_sep_v9.pdf}
% \vspace{-10pt}
% \caption{Parallel scaling of compute, where the x-axis shows K and the y-axis shows Pass@K and Maj@K accuracy on BrowseComp. For K2 and GLM-4.5, we first apply the Max \# Tool Call strategy, setting maximum tool usage to 30 and 50 respectively, then perform parallel scaling by independently sampling K = 1, 2, 4, 8, 16, 24, 32 trajectories. For Qwen3-2507, we apply the Max \# Tool Call strategy with a maximum of 15 tools, then apply Budget Forcing to add 15 more, followed by parallel scaling with K = 1, 2, 4, 8, 16, 24, 32 trajectories.
%         }
%         \label{fig:scaling_policy_pal}
%     \vspace{-15pt}

% \end{figure}


% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:different_passk}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budgetv1.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.6\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v5.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}

\paragraph{The Max \# Tool Call method underutilizes compute, while Budget Forcing boosts tool use and performance.} Figure~\ref{fig:scaling_policy_seq} illustrates how different models scale with test-time compute on BrowseComp under two methods: Max \# Tool Call and Budget Forcing. Under the Max \# Tool Call setting, even when models are allotted generous tool call quotas, they often terminate early. For instance, Qwen3-2507 shows diminishing returns—increasing its quota from 15 to 50 results in only marginal increases in tool usage and even performance drops. In contrast, Budget Forcing actively drives models to exploit available compute. After a single application of budget forcing, GLM-4.5's tool usage more than doubles, and its Pass@1 accuracy rises from 19\% to 27\%. Qwen3-2507 exhibits an even more pronounced jump, with its performance ceiling increasing from 8\% to 18\% across multiple rounds. However, we observe diminishing gains as the number of tool calls within a single trajectory increases. This saturation suggests that long trajectories challenge models to perform coherent long-range reasoning. 


\begin{figure}[t]
\vspace{-10pt}
        \centering
\includegraphics[width=0.98\textwidth]{iclr2026/fig/policy_model_performance_metrics_pal_sep_v9.pdf}
\vspace{-10pt}
\caption{Parallel scaling of compute, where the x-axis shows K and the y-axis shows Pass@K and Maj@K accuracy on BrowseComp. For K2 and GLM-4.5, we first apply the Max \# Tool Call strategy, setting maximum tool usage to 30 and 50 respectively, then perform parallel scaling by independently sampling K = 1, 2, 4, 8, 16, 24, 32 trajectories. For Qwen3-2507, we apply the Max \# Tool Call strategy with a maximum of 15 tools, then apply Budget Forcing to add 15 more, followed by parallel scaling with K = 1, 2, 4, 8, 16, 24, 32 trajectories.
        }
        \label{fig:scaling_policy_pal}
    \vspace{-15pt}

\end{figure}

% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis shows the number of K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:different_passk}
%     % \vspace{-10pt}
% \end{wrapfigure}
%To address this limitation, we turn to Parallel Scaling, which increases compute not by deepening single trajectories, but by sampling multiple independent ones.

% \subsection{Test-Time Compute Scaling Results}
% 2. Scaling Policy Compute
% 2.1 Agentic Scaffold 
% 2.2 Experimental Setup (Benchmark, Models, Evaluation Metrics)

% 2.3 Evaluation Results (no test time compute)

% 1. Test results of pass@1 for different models on the benchmark (max tool calls=15)
% 2. Scaling compute for GPT4.1/K2/GLM 4.5 on BrowseComp + GAIA using serial approach
% 3. Scaling compute for GPT4.1/K2/GLM 4.5 on BrowseComp + GAIA using parallel approach


% 2.4 Test-Time Compute Results


% \begin{wrapfigure}{r}{0.4\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget.pdf}\vspace{-10pt}
%     \caption{Pass@k of Mistral-24B based on the average results from AIME24 and AMC23. }
%     \label{fig:different_passk}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budgetv1.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budgetv2.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.6\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v5.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis shows the number of K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}
% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis represents K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies Parallel Scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}
\paragraph{Models exhibit strong exploration capabilities but struggle with exploitation.} As shown in Figure~\ref{fig:scaling_policy_pal}, surprisingly, increasing compute via parallel scaling leads to a rapid rise in Pass@K accuracy, indicating that with more sampled trajectories, models are increasingly likely to find at least one correct answer. For instance, GLM-4.5's Pass@K accuracy increases from 16\% to 67\% when scaling K from 1 to 32 on the extremely challenging BrowseComp benchmark. 
% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis represents K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies Parallel Scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}
% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis represents K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies Parallel Scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}
Figure~\ref{fig:combine_budget_parallel} in Appendix~\ref{sec:budget_forcing_parallel} further shows that combining Budget Forcing with parallel scaling enhances exploration even more. However, this does not translate into efficient exploitation: while K2 reaches a Pass@16 of about 34\%, its Maj@16 accuracy—reflecting the ability to identify the correct answer through majority voting—is only around 12\%. This gap suggests that simply encouraging broader exploration is insufficient. Instead, improving the model’s ability to recognize and select high-quality answers is critical. This suggests that instead of simply promoting more diverse exploration, we should focus on improving the model's ability to exploit promising candidates. In the following sections, we explore how incorporating external verification signals can improve exploitation efficiency in \textsection\ref{sec:scaling_verifier} and how balancing exploration with exploitation~\citep{zeng2024b,liu2024diving} leads to better overall performance in \textsection\ref{sec:heavy_version} .


% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v6.pdf}\vspace{-10pt}
%     \caption{A comparison of Qwen3-2507's performance after applying Max \# Tool Call and Budget Forcing followed by parallel scaling. The x-axis shows the number of K; the y-axis shows Pass@K and Maj@K. Max \# Tool Call limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \begin{figure}{t}{0.8\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v1.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{figure}


% \begin{figure}[t]
% \vspace{-10pt}
%         \centering
% \includegraphics[width=0.95\textwidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v1.pdf}
% \vspace{-10pt}
% \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.
%         }
%         \label{fig:combine_budget_parallel}
%     %\vspace{-10pt}

% \end{figure}

% \begin{wrapfigure}{r}{0.6\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget_sep_v5.pdf}\vspace{-10pt}
%     \caption{Budget Forcing in Parallel Scaling for Qwen3-2507. The x-axis shows the actual number of tool calls; the y-axis shows Pass@K and Maj@K. Tool Conditional limits tool usage to 15 calls and applies parallel scaling with K = 1, 2, 4, 8 independent trajectories. Budget Forcing increases this limit by 15 calls and uses the same K values.}
%     \label{fig:combine_budget_parallel}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \begin{wrapfigure}{r}{.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/policy_model_performance_metrics_pal_budget.pdf}\vspace{-10pt}
%     \caption{Pass@k of Mistral-24B based on the average results from AIME24 and AMC23. }
%     \label{fig:different_passk}
%     % \vspace{-10pt}
% \end{wrapfigure}

==> scaling_verifier.tex <==
\section{Scaling Verification Compute}
\label{sec:scaling_verifier}
In this section, we begin by introducing the \emph{asymmetric verification}, followed by the framework of the verifier we implemented. We then outline the experimental setup and present the results.



% 3. Scaling Verifier Compute
% 3.0 Asymmetry of Verification
% 3.1 Agentic Scafflod
% 3.2 Experimental Setup (Metrics)
% 3.3 Scaling Test-Time Compute
% 在Pass@8这个量级上研究scaling verifier compute的合理性，比就比Pass@16以及majority@16就可以




\subsection{Asymmetric Verification}
% The \emph{Asymmetry of Verification}~\citep{wei2025asymmetry} has become a central concept in AI, describing tasks where verifying a solution is significantly easier than generating one. \jh{this is not a good example as known answer and test cases are assumed to be given. I think here to follow the story in the abstract, also in the original Jason Wei's blog, that some tasks verification is more difficult, some tasks it is easier, and some tasks it is similarly difficult.}For example, given a known answer to a math problem or test cases for a coding task, it's straightforward to check whether a candidate solution is correct. Many recent works exploit this property to design rule-based reward systems for large-scale reinforcement learning, leading to major advances in reasoning models for challenging tasks like Olympiad math and competitive programming~\citep{guo2025deepseek,team2025kimi,seed2025seed1,luo2025deepscaler,zeng2025simplerl}. 

Asymmetric Verification has become a central concept in AI, highlighting tasks where verifying a solution is far easier than generating one. Many problems have this ``easy to verify'' property. For instance, in Sudoku or the Eight Queens problem, generating a valid solution requires extensive search, but once a candidate solution is given, verification is trivial by simply checking whether all constraints are satisfied. Some tasks, however, show near-symmetry of verification, where checking correctness takes almost as much effort as solving. A classic example is matrix multiplication: confirming the product of two large matrices is essentially as costly as performing the multiplication itself. At the other extreme, certain problems are hard to verify: writing code may be relatively straightforward, but rigorously verifying that it is free from security vulnerabilities can demand exhaustive formal verification or full security audits. This ``easy to verify'' property allows the construction of robust reward systems at relatively low cost. By leveraging inexpensive verification, AI performance can be significantly boosted through scaling during training or at test time.

The deep search task similarly exhibits this asymmetry. While forward search requires models to navigate a vast space and retrieve hard-to-find information—often through extensive exploration—verification only needs minimal effort to confirm whether a predicted answer satisfies the necessary conditions. Consider the following example from BrowseComp:

\begin{tcolorbox}[colback=blue!5!white, colframe=black]
Please provide the name of a video game released in 1992. The series' first game was featured in a globally recognized record book, and it earned a spot in an Australian photographer publication. The third game inspired a legacy sequel. The fifth installment was the first to have a Chinese dub.
\end{tcolorbox}
Given a video game, one can easily verify its validity via simple web searches by checking its release year, whether the first game was in the record book, and so on. We also evaluate different models on search and verification tasks across multiple benchmarks, measuring the number of tool calls each requires in Table~\ref{table:tool_call_number}. The results show that most deep research tasks exhibit asymmetric verification, and this asymmetry grows with task difficulty. For instance, in BrowseComp, GLM-4.5 uses about 75.3 tool calls to search for a candidate answer but only 18 tool calls to verify it. In this section, we aim to harness this asymmetry by introducing verifiers to filter candidate answers, thereby improving the efficiency of test-time compute usage.






\subsection{Overview of The Verifier Framework}
Our verifier shares the same design principles, framework, and search tools as the search agent in \textsection\ref{sec:search_agent_framework}, differing only in the system prompt. In the verifier’s prompt, the model is instructed to use search tools specifically to check the correctness of a predicted answer and to assign a confidence score based on whether the answer meets the necessary conditions confirmed by the search results. The full system prompt is provided in Figure~\ref{fig:verfier-prompt} in the Appendix.




% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/scaling_paretov2.pdf}\vspace{-10pt}
%     \caption{Best-of-8 and Weighted-of-8 (with verifier) against Maj@8 and Maj@16 (without verifier). The x-axis shows the actual number of tool calls, and the y-axis shows accuracy.}
%     \label{fig:verfier_advantage}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \subsection{Test-time Scaling Method}
% \jh{this section is repetitive}
% We can also expand verifier computation using sequential scaling or parallel scaling. Sequential scaling includes: (1) Tool Conditional Method: setting a limit in the system prompt on how many times the verifier can use the search tool. (2) Budget Forcing Method: after the verifier completes a verification, we grant it additional tool usage to discourage premature confidence scoring and prompt exploration of alternative verification paths or search strategies. Examples of budget forcing for verifiers are provided in the Appendix. Parallel scaling is simpler: for each predicted answer from the search agent, the verifier generates multiple independent verification trajectories. The final confidence score is the average across these trajectories, which helps reduce bias from any single sample.

% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/scaling_paretov1.pdf}\vspace{-10pt}
%     \caption{Best-of-8 and Weighted-of-8 (with verifier) against Maj@8 and Maj@16 (without verifier). The x-axis shows the actual number of tool calls, and the y-axis shows accuracy.}
%     \label{fig:scaling_policy_seq}
%     % \vspace{-10pt}
% \end{wrapfigure}


\subsection{Experimental Setup}
% Verifier computation can also be scaled sequentially (e.g., Budget Forcing) or in parallel, where multiple verification trajectories are generated for each candidate answer. The final confidence score is the average across trajectories, reducing bias from any single sample.
% We use the same open-source models introduced in \S ~\ref{sec:scaling_search_setup} and evaluate them on the most challenging benchmark, BrowseComp-en. To fairly compare the computational efficiency of scaling search agents versus scaling verifier agents, we start from the models in Figure ~\ref{fig:scaling_policy_pal} that have already undergone parallel scaling with K=8. From this baseline, we explore two directions: (1) further scaling the search agent’s computation—for example, increasing parallel sampling from 8 to 16 trajectories, corresponding to maj@8 → maj@16—and (2) introducing a verifier agent to evaluate the predicted answers from the existing K=8 trajectories. For the verifier-based approach, we filter candidates using the verifier’s confidence scores, testing strategies such as weighted-of-8 and best-of-8. We then compare the compute cost and performance gains of these two scaling methods.



We use the same open-source models introduced in \S\ref{sec:scaling_search_setup} and evaluate them on the most challenging benchmark, BrowseComp. To fairly compare the computational efficiency of scaling search agents versus scaling verifier agents, we start from the models that have already undergone parallel scaling. From this baseline, we explore two directions: (1) further scaling the search agent's computation, continuing to generate more trajectories through parallel sampling (2) introducing a verifier agent to evaluate the predicted answers from the existing trajectories. For the verifier-based approach, we filter candidates using the verifier's confidence scores, testing strategies such as Best-of-K and Weighted Voting. We note that verifier computation can also be scaled sequentially (e.g., Budget Forcing) or in parallel, where multiple verification trajectories are generated for each candidate answer. The final confidence score is the average across trajectories, reducing bias from any single sample.


\begin{table*}[t]
\centering

\caption{Average number of tool calls for searching and verification across models and benchmarks. Since xbench-DeepSearch has relatively simple search requirements and balanced difficulty between search and verification, we report only the tool calls needed for search.}
\vspace{-5pt}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{BrowseComp}} 
               & \multicolumn{2}{c}{\textbf{BrowseComp-zh}} 
               & \multicolumn{2}{c}{\textbf{GAIA}} 
               & \textbf{xbench-DeepSearch} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
& \textbf{Solve} & \textbf{Verify} 
& \textbf{Solve} & \textbf{Verify} 
& \textbf{Solve} & \textbf{Verify} 
& \textbf{Solve} \\ 
\midrule
Qwen3-2507 & 32.4 & 11.3 & 18.8 & 9.7 & 9.7 & 7.9 & 13.4 \\
K2        & 27.8 & 11.2 & 38.2 & 6.3 & 6.2 & 5.8 & 2.9  \\
GLM-4.5    & 75.3 & 18.0 & 48.3 & 9.0 & 17.4 & 10.6 & 6.1 \\
\bottomrule
\end{tabular}

}
% \vspace{-5pt}
% \caption{Average number of tool calls for searching and verification across models and benchmarks. Since xbench-DeepSearch has relatively simple search requirements and balanced difficulty between search and verification, we report only the tool calls needed for search.}
\label{table:tool_call_number}
\vspace{-15pt}
\end{table*}


\subsection{Experimental Results}


% \begin{table*}[t]
% \centering
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{BrowseComp}} 
%                & \multicolumn{2}{c}{\textbf{BrowseComp-zh}} 
%                & \multicolumn{2}{c}{\textbf{GAIA}} 
%                & \textbf{xbench-DeepSearch} \\ 
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
% & \textbf{Solve} & \textbf{Verify} 
% & \textbf{Solve} & \textbf{Verify} 
% & \textbf{Solve} & \textbf{Verify} 
% & \textbf{Solve} \\ 
% \midrule
% Qwen3-2507 & 32.4 & 11.3 & 18.8 & 9.7 & 9.7 & 7.9 & 13.4 \\
% K2        & 27.8 & 11.2 & 38.2 & 6.3 & 6.2 & 5.8 & 2.9  \\
% GLM-4.5    & 75.3 & 18.0 & 48.3 & 9.0 & 17.4 & 10.6 & 6.1 \\
% \bottomrule
% \end{tabular}

% }
% \caption{Average number of tool calls for searching and verification across models and benchmarks. Since xbench-DeepSearch has relatively simple search requirements and balanced difficulty between search and verification, we report only the tool calls needed for search.}
% \label{table:tool_call_number}
% \vspace{-10pt}
% \end{table*}

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/fig5_merge.pdf}\vspace{-10pt}
%     \caption{Best-of-8 and Weighted-of-8 (with verifier) against Maj@8 and Maj@16 (without verifier). The x-axis shows the actual number of tool calls, and the y-axis shows accuracy.}
%     \label{fig:verfier_advantage}
%     % \vspace{-10pt}
% \end{wrapfigure}

\begin{figure}[!t]
        \centering
\includegraphics[width=0.97\columnwidth]{iclr2026/fig/fig5_mergev2.pdf}
 \vspace{-5pt}
\caption {Parallel scaling results of different models on BrowseComp.  The x-axis shows the number of tool calls counting both the searcher and the verifier. The solid lines represent the growth of Maj@K corresponding to scaling the searcher's compute, while the dashed lines represent the growth of Best-of-K and Weighted Voting after introducing a verifier.} 
        \label{fig:verfier_advantage}
\end{figure}

\paragraph{Verifier yields superior accuracy–cost trade-off.} 
% \jh{this paragraph and figure 5 are missing the point, the most important point of this paragraph should be emphasizing asymmetry, which is one central point of the paper. However, this paragraph does not mention it at all. To reflect asymmetry, I also feel figure 1-like figure is more clear than the current figure 5.}Figure~\ref{fig:verfier_advantage} illustrates the accuracy of candidate answer selection—based on eight independently sampled trajectories from the search agent—when filtered through the verifier, under both best-of-8 and weighted-of-8 strategies. Rather than further scaling the search agent’s computation, augmenting it with a verifier delivers comparable or even superior accuracy at a fraction of the cost. For example, with GLM 4.5, verifier-based selection reaches an accuracy of nearly 0.4 on BrowseComp-en—matching Maj@16—while requiring only about 20\% of the compute\jh{when describing the restuls, let's describe the fact and use number of tool calls rather than compute, while we can say in different places that the number of tool calls is a close mirror of compute}. Likewise, for K2, the verifier attains around 0.18 accuracy with only half the compute, surpassing Maj@16 by a clear margin.
Figure~\ref{fig:verfier_advantage} illustrates that the asymmetry property of verification consistently appears across different models when scaling test compute. In other words, adding a verifier allows accuracy to grow more quickly than simply increasing the computation of the search agent. For example, with GLM-4.5, increasing search computation alone requires about an additional 560 tool calls just to raise accuracy from 35.7\% with Maj@8 to 40.8\% with Maj@32. By contrast, introducing a verifier achieves a larger gain with far less cost: only about 100 additional tool calls are needed to improve from 35.7\% with Maj@8 to 45\% with Weighted Voting. A similar pattern emerges with K2. Without a verifier, raising performance from around 10\% with Maj@8 to 15.2\% with Maj@32 requires an increase of about 370 tool calls. With a verifier, however, the same starting point improves to 18\% with Best-of-8 or Weighted Voting after only about 77 additional tool calls.



% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/scaling_paretov2.pdf}\vspace{-10pt}
%     \caption{Best-of-8 and Weighted-of-8 (with verifier) against Maj@8 and Maj@16 (without verifier). The x-axis shows the actual number of tool calls, and the y-axis shows accuracy.}
%     \label{fig:verfier_advantage}
%     % \vspace{-10pt}
% \end{wrapfigure}


% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/scaling_paretov1.pdf}\vspace{-10pt}
%     \caption{Best-of-8 and Weighted-of-8 (with verifier) against Maj@8 and Maj@16 (without verifier). The x-axis shows the actual number of tool calls, and the y-axis shows accuracy.}
%     \label{fig:scaling_policy_seq}
%     % \vspace{-10pt}
% \end{wrapfigure}

\paragraph{Scaling the verifier can further raise the performance ceiling, though the gains depend on the model and strategy used.} We apply the scaling methods like  Max \# Tool Call, Budget Forcing and Parallel Scaling to the verifier, with results shown in Figure~\ref{fig:policy_verifier_scaling_comparison}. These methods lead to notable improvements. For example, in the K2 case, applying Budget Forcing increases actual tool usage and boosts accuracy from 10\% to 20\%.
% We apply the scaling methods like  Max \# Tool Call, Budget Forcing and Parallel Scaling to the verifier, with results shown in Figure~\ref{fig:policy_verifier_scaling_comparison}. The Max \# Tool Call method still provides initial accuracy gains, but in some cases, increasing the tool usage quota does not lead to greater actual tool use and can even reduce performance. For example, in the K2 case, increasing the quota from 30 to 50 tools has little impact on actual usage, while both Best-of-8 and Weighted Voting accuracy drop from 18\% to 14\%. In contrast, applying Budget Forcing successfully raises actual tool usage and improves Best-of-8 accuracy from 18\% to 20\%.
% For example, on Qwen3, Budget Forcing increases tool usage from [ ] to [ ], and boosts best-of-8 accuracy from [ ] to [ ].
% \paragraph{Verifier scaling is model- and strategy-dependent.} Performance gains from scaling verifier computation vary substantially across models and strategies. Different scaling methods—such as budget forcing or parallel scaling—and answer selection schemes—such as best-of-n or weighted-of-n—yield distinct improvement patterns. For example, with GLM 4.5, parallel scaling combined with the best-of-8 approach achieves a higher gain, reaching 0.42 on BrowseComp-en. In contrast, for K2, budget forcing delivers better best-of-8 performance with lower computational cost. These results indicate that in practical applications, scaling strategies should be chosen with careful consideration of both model characteristics and available compute, to maximize performance per unit of computation.
Scaling methods such as budget forcing or parallel scaling, and answer aggregation schemes such as Best-of-N or Weighted Voting produce distinct improvement patterns. For example, with GLM-4.5, parallel scaling paired with the Best-of-8 approach achieves the largest gain, reaching 42\% on BrowseComp. In contrast, K2 attains better Best-of-8 accuracy with lower compute using budget forcing. These results show that, in practical deployments, the choice of scaling target (e.g., search agent or verifier agent), scaling strategy, and answer aggregation metric should be guided by both the model’s characteristics and the available compute budget, to maximize performance per unit of cost. 

%These results highlight that practical deployments should select scaling strategies based on both model characteristics and compute constraints to maximize performance per unit cost.

\begin{figure}[!t]
        \centering
\includegraphics[width=0.97\columnwidth]{iclr2026/fig/qwen_k2_glm4.5_comparison_v6.pdf}
% \vspace{-10pt}
\caption {Different strategies for scaling verifier computation across models. The top panel shows accuracy, and the bottom panel shows the corresponding number of tool calls. Along the x-axis, vanilla indicates the Maj@8 accuracy achieved by scaling the search agent without verification, while Max \# Tool Call, Budget Forcing, and Parallel Scaling show the Best-of-8 results when applying these strategies to increase verifier compute.}
        \label{fig:policy_verifier_scaling_comparison}
\vspace{-15pt}
\end{figure}

